RPT: Relational Pre-trained Transformer Is Almost All You Need towards Democratizing Data Preparation

Can AI help automate human-easy but computer-hard data preparation tasks that burden data scientists, practitioners, and crowd workers? We answer this question by presenting RPT, a denoising auto-encoder for tuple-to-X models (X could be tuple, token, label, JSON, and so on). RPT is pre-trained for a tuple-to-tuple model by corrupting the input tuple and then learning a model to reconstruct the original tuple. It adopts a Transformer-based neural translation architecture that consists of a bidirectional encoder (similar to BERT) and a left-to-right autoregressive decoder (similar to GPT), leading to a generalization of both BERT and GPT. The pre-trained RPT can already support several common data preparation tasks such as data cleaning, auto-completion and schema matching. Better still, RPT can be fine-tuned on a wide range of data preparation tasks, such as value normalization, data transformation, data annotation, etc. To complement RPT, we also discuss several appealing techniques such as collaborative training and few-shot learning for entity resolution, and few-shot learning and NLP question-answering for information extraction. In addition, we identify a series of research opportunities to advance the field of data preparation.

==> response/general.tex <==
%!TEX root = ../paper.tex
\subsection*{\mbox{Dear VLDB Meta-Reviewer and Reviewers,}}

\vspace{1ex}
We thank the meta-reviewer and reviewers for the constructive reviews and encouraging comments on our vision paper  ``{\em \system: Relational Pre-trained Transformer Is Almost All You Need towards Democratizing Data Preparation}''.
We have made a major revision to significantly improve the paper and have better framed our vision based on these valuable comments. The revised parts are highlighted in \add{blue} in this revision.

==> response/meta.tex <==
%!TEX root = ../paper.tex
\subsection*{Response to the Meta-Reviewer}

\stitle{\fbox{Required Items.}} \\
{\em
R1. Better justification of the design choices and of the insights; \\
R2. Enhancing the related work by adding several missing references.
}

\vspace{1ex}
\stitle{[{\em Response}]}
We have addressed all comments of each individual reviewer and significantly revised the paper. The major changes are listed below.

\bi
	\item {\em Paper Re-organization.}
	To remove the confusions introduced in the original submission by defining different models for different data preparation tasks (\ie~\system-C for data cleaning, \system-E for entity resolution, and \system-I for information extraction), we have made the following  changes:
	\bi
		\item We have defined a unified Transformer-based sequence-to-sequence model \system, for general purpose tuple-to-tuple pre-training. (Section~\ref{sec:rpt-model})
		
		\item We have added a discussion about how \system can be fine-tuned to serve many data preparation tasks, beyond data cleaning, entity resolution and information extraction. (Section~\ref{sec:finetune})

		\item We have merged the previous discussion about ER and IE and discussed how other techniques can  complement RPT in these two tasks. (Section~\ref{sec:beyond})
	\ei

	\item {\em R1: Better justification.}
	We have added better justifications about {\em what is the goal of \system} and {\em how \system works} at the following places:
	\bi
		\item Abstract: \system is a denoising autoencoder for {\em tuple-to-X} models (``$X$'' could be tuple, token, label, JSON, and so on).
		\item Section~\ref{sec:intro}: revised ``Scenarios'' 1--2, ``Desiderata'', and ``RPT Is Almost All You Need''.
		\item Section~\ref{sec:rpt-model}: the choice of the \system architecture (Section~\ref{subsec:rpt-architecture}), and the tuple-aware ``Token Masking'' (Section~\ref{subsec:rpt-pretrain}).
		\item Section~\ref{sec:finetune}: fine-tuning \system for many common data preparation tasks, \ie from {\em tuple-to-tuple} to {\em tuple-to-X}.
	\ei
	\item {\em R2: Enhancing Related Work.}
	We have enhanced related work at the following places:
	\bi
		\item Section~\ref{subsec:rpt-related}: we have added discussion and related work for {\em Knowledge Bases} and {\em Relational Table Understanding}.
		\item Section~\ref{subsec:rpt-e}: we have added the paper~\cite{DBLP:conf/edbt/BrunnerS20} that compares different pre-trained models, as suggested.
	\ei
\ei

==> response/r1.tex <==
%!TEX root = ../paper.tex
\subsection*{Responses to Reviewer \#1}

\stitle{\fbox{R1W1.}} 
{\em There is very limited discussion for the human-in-the-loop within the proposed framework.}


\stitle{\fbox{R1D1.}} 
{\em One area that could see a stronger focus is the human-in-the-loop. Clearly, many of the discussed tasks and examples will require human intervention at some point (e.g., to decide between a given set of choices for replacing a missing value). If I look at the question Q2 (``The city for the Michael Jordan with expertise in Basketball''), for example, my intuitive answer would have been Chicago or maybe Charlotte. And even if the question is reformulated to ``the birth place for ...'' I would have to think a bit about whether to put New York City or Brooklyn. I understand that this is just one example but I argue that some of these tasks are not as easy even for a human. They often require additional context and expertise. So, these automated models are likely to make mistakes. Would I really want to prepare my data using a model that potentially introduces new errors or be in control (e.g., answer a few questions here and there where the model is uncertain)? The authors mention the possibility of multiple answers at some point. Limiting the involvement of the user and learning from their decisions (e.g., active learning as briefly mentioned in the paper) seems like an important goal for a (semi-)automated data preparation system. To me there is additional opportunity/need to investigate how to interact with the user and potentially incorporate feedback into the algorithms. This would also further distinguish the proposed system from the existing work.}


\vspace{1ex}
\stitle{[{\em Response to R1W1 \& R1D1}.]}
We fully agree with the reviewer that the concept of human-in-the-loop is critical for data preparation. 
Although our proposal \system is a pre-trained model that can be either directly used or fine-tuned before being used, there is a natural connection between \system and human-in-the-loop. We have further emphasized this connection at the following places.

\bi
	\item Section~\ref{subsec:rpt-opp} ``Opportunities'' (O3): it is practical to consider \system as an AI-assistant for many human-in-the-loop data preparation tasks, where \system can provide suggestions, through which to actually reduce human cost.
	%
	Actually, in our motivating Scenario 1 in Section~\ref{sec:intro}, the auto-completion and auto-suggestion cases already have human-in-the-loop.

	\item Section~\ref{subsec:rpt-e} ``Entity Resolution'': we have further emphasized in several places the necessity of human-in-the-loop, including ``Consolidator'', ``Vision and Opportunities'' (the 2nd and 3rd paragraphs, and (O2) ``Few-shot learning'').

	\item Section~\ref{sec:rpt-i} ``Information Extraction'': as motivated in Figure~\ref{fig:rpt-i}, such tasks are typically performed by crowd workers (or crowd-in-the-loop). Instead of fully replacing crowd workers, we plan to train multiple  AI-workers (or AI-turkers), and mix the AI-workers and crowd workers to reduce the total cost of a crowdsourcing task. 
\ei


\stitle{\fbox{R1W2.}} 
{\em Learning from dirty data.}

\stitle{\fbox{R1D3.}}
{\em The challenge of learning from dirty data is also only briefly discussed. Many of the publicly available dataset are likely to contain some low quality data, e.g., typos during data entry, or will require some normalization, e.g., ST vs. STREET for address data. The effectiveness of an automated data preparation system is strongly dependent on being able to learn from such dirty data.}

\stitle{[{\em Response to R1W2 \& R1D3}.]}
This is an important observation and one that is frequently discussed in different fora, either in Academia or Industry. 
In the case of RPT, we are faced with the following practical situation: 
On the one hand, we cannot afford to clean the huge collection of tables we are learning from; on the other hand, feeding RPT with dirty risks to produce bad models (``garbage-in, garbage-out''). 

It is well understood that language models (\eg GPT-3) are usually fed with data from different, not necessarily curated, corpora, such as the common crawl, and still achieve outstanding results in different tasks.
Analogously, \system is facing a similar situation as GPT-3, with the difference that RPT learns from (dirty) tuples.
Our assumption for RPT is that data tables are not ``very'' dirty and that the model should be robust to low error rates and it will be able to pickup  enough ``good'' redundancies in the data to be useful in the three applications of RPT.  
As a simple example, if  ``\at{Micheal} Jordan'' (where ``Micheal'' is a typo) for the UC Berkeley professor appears only once in our training tables, 
the model will learn the wrong name. 
However, if ``Micheal Jordan'' appears only once and ``Michael Jordan'' appears many more times, then most likely the model will provide the correct answer. 
This case is similar to ``ST'' and ``STREET'', if the model needs to make a choice between one of them, the model will pick the one with a higher probability, \ie the one that it sees more times during the training process.
To mitigate the  bad effects of dirty data, RPT could follow a similar approach to the one performed by GPT-3, namely filtering the input data using a corpus of trusted data, and deduplication through simple similarity-based filtering, similar to what has been done for text corpora (see~Appendix A in~\cite{DBLP:journals/corr/abs-2005-14165} for details). 


We have clarified in Section~\ref{subsec:rpt-exp} for pre-training \system, and in Section~\ref{subsec:rpt-e} for collaboratively training an entity resolution Matcher, that in the current setting we learn directly from dirty data. 

We have also clarified in Section~\ref{subsec:rpt-opp} ``Research Opportunities (O2) that
(i)~we learn from dirty data; (ii)~we assume that the frequency of correct values is much higher than the frequency of wrong values, an assumption that mostly holds in practice; and (iii)~how to improve the model robustness while learning from dirty data is an important research direction, and it is important to build a high quality training dataset, similar to the Colossal Clean Crawled Corpus (C4) for Text-To-Text-Transfer-Transformer (T5)~\cite{t5}.
%
Moreover, we include the need for high quality training dataset in Section~\ref{sec:conclusion} ``Call to Arms''.


\stitle{\fbox{R1W3.}} 
{\em The issue of loading and transforming data into a common representation is largely ignored.}

\stitle{\fbox{R1D4.}} 
{\em I wonder whether the focus is on the right data preparation tasks. It is true that data preparation is a time consuming task. However, in many cases the issues that a user has to deal with are more at the lower level. For example, loading data in different formats and transforming it into some standardized representation, and standardization of values before using them as input for data analysis. These tasks should at least be included in the framework if the goal is to democratize data preparation.}


\stitle{[{\em Response to R1W3 \& R1D4.}]}
We fully agree with the reviewer that data preparation covers a plethora of tasks including those mentioned by the reviewer, as well as many others as addressed in the literature~\cite{DBLP:journals/sigmod/HameedN20, Cezhang2021, DBLP:conf/cidr/DengFAWSEIMO017, DBLP:journals/pvldb/AbedjanCDFIOPST16} and white papers from the industry~\cite{gartnerdataprep2020}. 

We have revised the scope of \system to better justify that it is designed to cover many common data preparation tasks.
In particular, we have clarified the generality of \system at the following places:

\bi
	\item {\em Abstract}: 
	\system is a Transformer-based encoder-decoder architecture for {\em tuple-to-X} models (``$X$'' could be tuple, token, label, JSON, and so on). \system is pre-trained for a {\em tuple-to-tuple} model by corrupting the input tuple and then learning a model to reconstruct the original tuple, but it can be fine-tuned for different output formats (\ie the format of {\em X} in {\em tuple-to-X} can be easily extended). This is because of the flexibility provided by \system's encoder-decoder architecture that can support neural translation from one type of input (\eg tuples) to many other types of output.
	Clearly, more data preparation tasks than what have been discussed in this paper can be supported through fine-tuning \system.

	\item {\em Section~\ref{subsec:rpt-opp}, the 1st paragraph}: 
	The pre-trained \system can directly support several common data preparation tasks, such as error detection, data repairing, auto-completion, auto-suggestion, and schema matching.
	This is because the way  the masked training of \system works; we mask (1) attribute name, (2) entire attribute values, and (3) single attribute value, as discussed in Section~\ref{subsec:rpt-pretrain} ``Token Masking''.

	\item {\em Section~\ref{sec:finetune}, Fine-tuning \system}: 
	The bidirectional encoder and the left-to-right autoregressive decoder  allows  \system to be fine-tuned  for many downstream data preparation tasks, such as value normalization, data transformation, data annotation, information extraction, etc. 
\ei

\stitle{\fbox{R1W4.}} 
{\em The distinction to some of the existing work should be clearer.}


\stitle{\fbox{R1D5.}} 
{\em The discussion of related work needs to be deeper at some points. In particular with respect to TURL which seems to also address two of the discussed data preparation tasks (entity linkage and cell filling) plus additional tasks (row population and schema augmentation). It is not completely clear to me what ``learning more human-readable knowledge'' means and why a focus on wider tables is necessary.}


\stitle{[{\em Response to R1W4 \& R1D5.}]}
Thank you for the suggestion. We have added a discussion about the differences in Section~\ref{subsec:rpt-related} ``Related Work''.
Below, we provide a detailed explanation about the fundamental differences between  \system and TURL:

\sstab
%{\emph{(1) Differences in application scenarios.}}
%\mourad{not sure we're talking about application scenarios here}
{\emph{(1) Differences in learning goals and assumptions.}}
TURL focuses on learning representations of entities in an existing knowledge base (KB) via pre-training. 
Then, when serving down-streaming tasks (\eg cell filling), TURL needs to employ both (i) a pre-trained model and (ii) a collection of entities in the KB, 
where the total size is 1.2 GB for the pre-trained model and 4.7 GB for the KB\footnote{We have confirmed with the first author of TURL that a KB is needed when using (not only training) TURL for prediction, which is a big collection of web tables.}, as found in their public code repository.
In contrast, \system focuses on learning relationships within tuples. 
In particular, \system only utilizes a pre-trained model, which takes around 1.6 GB in our experiment.

%Next, we elaborate on the differences using the example $Q_1$ in our sample data cleaning task shown in Figure~\ref{fig:scenarios}(a).
In addition, \system  and TURL make different assumptions. More specifically,  using the example $Q_1$ in our sample data cleaning task shown in Figure~\ref{fig:scenarios}(a):

\bi
	\item TURL assumes that the dependency between the subject  (\eg \at{name}) and object columns (\eg \at{expertise} and \at{city}) is \emph{given}. 
	To fill in the missing value in $\at{city}$, it predicts which entity in the KB should be associated with subject entity \at{Michael~Jordan} based on the surrounding entity cells and meta-data. After that, it extracts the name of the predicted entity from the KB (or web tables) to fill in the cell.

	\item In contrast, \system {\em neither} assumes the dependency between subject and object columns is given, {\em nor} utilizes an existing KB. Instead, \system automatically captures column dependencies in the pre-training phase and recovers the missing cell based on other cells in the tuple in the prediction phase.
\ei

\sstab
{\emph{(2) Differences in model design.}}
%Technically, we describe 
The differences in the design principles of TURL and \system are as follows.

\bi
	\item {\em Model Architectures}.
	\bi
		\item TURL employs an \emph{encoder}-only architecture that takes an \emph{entire} table as input to learn contextual representation.
		
		\item \system adopts an \emph{encoder-decoder} architecture, which has been empirically proved to outperform the encoder-only architecture 
		for many NLP tasks by Google T5~\cite{t5} and BART~\cite{bart}.
	\system first uses a bi-directional Transformer (\ie encoder) to learn a representation of a dirty (\ie corrupted) \emph{tuple}, rather than the entire table.  Then, it feeds the representation to an auto-regressive Transformer (\ie decoder) to reconstruct the original (\ie correct) tuple. Furthermore, the auto-regressive Transformer-based decoder can be fine-tuned to generate other types of outputs (see Section~\ref{sec:finetune}). 
	\ei

	\item {\em Pre-training Tasks}.
	\bi
		\item TURL uses two pre-training tasks: (i)~masked language model (MLM) on \emph{meta-data}, e.g., caption and headers, and (ii)~masked entity recovery on cells.
		The latter is designed for recovering the \emph{linked} entity in the KB based on the surrounding entity cells and meta-data.
		\item \system employs Attribute Name and Attribute Value Masking (see Section~\ref{subsec:rpt-pretrain} ``Token Masking'') that directly recovers an attribute name or value in a tuple.
	\ei
\ei

\sstab
{\emph{(3) Empirical comparison.}}
We also conduct a new experiment to compare TURL and \system. 
To this end, we extracted $1221$ web tables from the dataset used in TURL for pre-training, where each table contains columns regarding \at{city} and \at{country}. 
Different from TURL, we only use headers as meta-data, and do not assume that the dependency between subject and object columns is given.

After pre-training, we employ TURL and \system to fill in missing values in \at{country} and compare their results. %We have the following experimental findings.
On the one hand, for $736$ test tables, TURL cannot find the subject entity in the KB and thus returns empty results, while \system can achieve $0.75$ accuracy. 
On the other hand, for $1,075$ tables, TURL can find subject entities in the KB and obtained $0.64$  accuracy, while \system achieves $0.69$. 
Overall, the accuracy scores of TURL and \system are $0.48$ and $0.71$, respectively. The results show that \system can achieve better performance 
on cleaning relational tables with no assumptions on column dependency and no external knowledge.


\stitle{\fbox{R1D2.}} 
{\em The proposal focuses on solutions that ``Search the Data Ocean'' (Type III). A lack of rich metadata, however, is often one of the main problems with data preparation tasks. As such it seems that generating and managing such metadata (e.g., using a Knowledge graph) is a more viable or at least equally important solution. Going back to Q2. A system that learns on player statistics data (which is likely to be more abundant than other information about the players) would likely return the city (cities) of the team(s) that the player played for during their career. Without additional metadata there is always a high risk for false predictions. A component for learning and maintaining such metadata is another important challenge.}


\stitle{[{\em Response to R1D2.}]} 
We agree that maintaining meta-data, e.g., using a knowledge graph, is also important and promising, as pointed out by the reviewer.
We would like to differentiate between a knowledge graph and a pre-trained deep learning model, which is adopted in this paper, in terms of the knowledge they hold:

\bi
	\item {\em Explicit knowledge.}
	Knowledge graphs  represent ``explicit knowledge'' that is extracted from different data sources and oftentimes curated using different methods, usually based on heuristics.
	They are widely used in many companies such as Google, Amazon, Microsoft, and so on.

	\item {\em Implicit knowledge.}
	Pre-trained deep learning models represent ``implicit knowledge'', which is learned through a neural network trained on a large corpus of data, and which can be used in many tasks but  oftentimes without much explanations. A prime example is GTP-3.
\ei

Then, 
we want to clarify that there are pros and cons for each approach as follows.
%and both are important and promising, as pointed out by the reviewer. 

\bi
	\item {\em Knowledge graphs (KGs):} the explicit knowledge.
	\bi
		\item Building and maintaining high-quality KGs are time consuming and they often require human efforts. 
		For example, Google knowledge graph needs manual check for the information about important persons such as Joe Biden, but uses automatic algorithms to build or maintain for those persons in the long tail.
		\item KGs do not normally have enough coverage.
		\item Using KGs for table understanding and table annotation cannot be fully automatic; these would need to first match tuples in tables to subgraphs in knowledge graphs, and humans are needed to confirm both the matching relationship and which values to change~\cite{DBLP:conf/sigmod/ChuMIOP0Y15}.
	\ei
	\item {\em Pre-trained deep learning models:} the implicit knowledge.
	\bi
		\item They may not be as accurate as using well-curated knowledge graphs.
		\item They are usually not explainable. 
	\ei
\ei


We have now clarified the difference of these two options in Section~\ref{subsec:rpt-related} ``Knowledge bases''. %, and have pointed out that combining explicit knowledge and implicit knowledge is an interesting research topic.
We have also discussed the importance of explainable AI techniques for assisting deep learning models such as \system.

\stitle{\fbox{R1 Typos.}} \\
{\em Can be build GPT-3 like models for relational data? (page 2) \\
... so we can directly compared with state-of-the-art ZeroER (page 6)}


\stitle{[{\em Response}]}
Fixed. Thanks!

==> response/r2.tex <==
%!TEX root = ../paper.tex
\subsection*{Responses to Reviewer \#2}

\stitle{\fbox{R2W1.}} 
{\em The title is a bit imprecise. The paper discusses mostly how to fine-tune pre-trained language models for data preparation tasks, instead of how to pre-train a transformer model from scratch for relational data. The title could be more precise about this.}

\stitle{\fbox{R2D1.}} 
{\em To use pre-trained LMs for tasks on relational tables, existing approaches are in two different directions: 1). fine-tune pre-trained LM base with tasks-specific objectives, e.g., Ditto, 2). pre-train a transformer from scratch with global self-training objectives and then fine-tuned by task-specific objectives, e.g., TURL. A key benefit of the second direction is that the model can learn task-agnostic features from the global self-training objectives, which can further benefit downstream tasks. However, the distinctions between global (task-agnostic) self-training objectives and local (task-specific) self-training objectives are not explicitly discussed in the paper.}


\stitle{[{\em Response to R2W1 \& R2D1.}]}
This is a discerning point! We have significantly restructured the paper to make this point clear. We have also changed the paper title to ``\system: Relational Pre-trained Transformer Is Almost All You Need towards Democratizing Data Preparation'' based on your comment R2D3, to better align the title with the revised paper content.
%
In particular, we have removed the previous confusion about different models (\ie~\system-C for data cleaning, \system-E for entity resolution, and \system-I for information extraction), with the following changes:

\bi
	\item We have revised Abstract to better frame our proposal.

	\item We have defined a unified Transformer-based sequence-to-sequence model \system, for general purpose tuple-to-tuple pre-training. (Section~\ref{sec:rpt-model})
	
	\item We have added a discussion about how \system can be fine-tuned for many data preparation tasks, besides information extraction and entity resolution. (Section~\ref{sec:finetune})

	\item We have merged the previous discussion about entity resolution and information extraction, in order to discuss what other appealing techniques can help. (Section~\ref{sec:beyond})
\ei

\stitle{\fbox{R2W2.}} 
{\em While the authors briefly mention collaborative training and MLM in the intro, it is not clear how to transfer knowledge acquired from one task, e.g., data cleaning, for another task, e.g., entity matching.}

{\em The paper discusses three independent architectures for three data preparation tasks. Thus, knowledge is not shared between different tasks. The authors can consider adding discussions about whether it is beneficial to share knowledge and how to share knowledge learned from different tasks.}

\stitle{[{\em Response to R2W2 \& R2D2.}]}
We have clarified in the revised version that, by better aligning \system to the pre-training/fine-tuning paradigm (see our response to R2W1 \& R2D1), it is evident that learned knowledge can be shared. More concretely:


\bi
	\item Pre-trained \system (Section~\ref{subsec:rpt-opp}): the pre-trained \system can directly support error detection, data repairing, auto-completion, auto-suggestion, and schema matching.

	\item Fine-tuning \system (Section~\ref{sec:finetune}): besides discussing its connection with information extraction and entity resolution, we also discuss how to fine-tune \system for value normalization, data transformation, and data annotation.
\ei
 

\stitle{\fbox{R2W3.}} 
{\em Lack of discussion about the limitations of pre-trained LMs.}

\stitle{\fbox{R2D3.}} 
{\em Limitations of pre-trained LMs. There certainly many limitations about pre-trained LMs, so it is more precise to say ``Relational Pretrained Transformers (RPTs) are *almost* All You Need''. \\
1). Numeric values. Due to the vocabulary size of existing pre-trained LMs (e.g., BERT and BART), many numeric values are mapped into unknown tokens in the tokenization phase. Thus, the model will fail on tasks that require precise prediction on numeric values. \\
2). Max sequence length. Restricted by the GPU memory size, most pre-trained LMs are limited by the sequence length, thus data preparation on large tables may require additional optimization. \\
3). Shifted domain and vocabulary. Existing pre-trained LMs are trained with open domain text and are designed for natural language tasks. Thus, the vocabulary of such models is determined by the open-domain textual data. However, the vocabulary of relational tables could be very different with textual data. This is related to D1. TURL builds the vocabulary from scratch, thus will suffer less from this problem.
}

\stitle{[{\em Response to R2W3 \& R2D3.}]}
Great points! We have added a discussion about limitations at the end of Section~\ref{subsec:rpt-exp}.

Also, we take the cool suggestion to add the *almost* to ``Relational Pre-trained Transformer (RPT) Is All You Need'' in Section~\ref{sec:intro}. 


\stitle{\fbox{R2D4.}} 
{\em D4. Minor points. \\
1). Experiment settings of RPT-C. For the pre-training phase, it is not clear whether Abt-Buy and Walmart-Amazon are clean or dirty. \\
2). Table2 should include results that also leverage pre-trained models, e.g., Ditto, TURL, or Brunner et.al.
Brunner, Ursin, and Kurt Stockinger. ``Entity matching with transformer architectures-a step forward in data integration.'' EDBT, Copenhagen, 30 March-2 April 2020. 2020.
Although the reported results from these papers use different settings, i.e., their training/test sets are from the same table, it is easy to re-train these models using the same ``trained on other benchmarks'' setting. \\
3). Using a seq2seq model for data correction could be an error-prone process. Most pre-trained seq2seq models, e.g., BART, T5, or Pegasus, won't obtain perfect reconstruction performance. Thus, directly using a single seq2seq model for both error detection and error correction tasks can easily corrupt correct values. \\
4). Other related papers:
Yin, Pengcheng, et al. ``TaBERT: Pretraining for Joint Understanding of Textual and Tabular Data.'' arXiv preprint arXiv:2005.08314 (2020).
Chen, Wenhu, et al. ``TabFact: A large-scale dataset for table-based fact verification.'' arXiv preprint arXiv:1909.02164 (2019).
}


\stitle{[{\em Response to R2D4.}]}
(1) We did not clean the tables used for training. We have clarified this point in Section~\ref{subsec:rpt-exp} ``Preliminary Results'', the first paragraph.

\stab
(2) Thank you for the suggestion.
We have added a new experiment to compare our approach with the pre-trained model, Ditto, and included the results in Table~\ref{tbl:rpte-expt}. 
The results show that our approach uses \at{zero} example from the test ER dataset to achieve the performance of Ditto, which is trained by fine-tuning BERT with 1000+ examples.
This is because the collaborative learning method can enable the knowledge learned and transferred from one dataset to other datasets, and thus reduce the human cost of data annotation.
More details can be referred to Section~\ref{subsec:rpt-e} ``Preliminary Results''.
We also note that the EDBT paper~\cite{DBLP:conf/edbt/BrunnerS20} is quite similar to Ditto. First, both studies use the same strategy to model a record pair as a sequence and fine-tune a pre-trained model to output the matching results. Second, the EDBT paper~\cite{DBLP:conf/edbt/BrunnerS20} compares different pre-trained LM models for entity resolution and reports that RoBERTa achieves the best performance. Similarly, the latest version of Ditto~\cite{DBLP:journals/corr/abs-2004-00584} also uses RoBERTa as its pre-trained model. Third, both studies achieve similar results in the experiments. For example, on the Abt-Buy dataset, the EDBT paper and Ditto achieve $0.91$ and $0.90$ on F1 score respectively.


%
%Generally speaking, deep learning for entity matching has two steps: (i) use a pre-trained model $f()$ to convert an entity $e$ to an embedding $v_e$, \ie $v_e = f(e)$; and (2) given two embeddings $v_{e_1}$ and $v_{e_2}$, train a matcher $M()$ to decide match or not, \ie $M(v_{e_1}, v_{e_2}):$ true or false.
%
%Note that when comparing with Ditto, we use BERT instead of \system, to generate representations because the purpose of this experiment is to test whether collaborative learning works at all, by using the same entity representations (\ie fixing $f()$).
%
%The purpose of the comparison with Ditto is that: if we fix the function $f()$, whether our proposed collaborative training can help pre-train the matcher $M()$ without using any labeled data from the current ER task, for which we fix the function $f()$ to be BERT. 
%
%On the other hand, the EDBT paper~\cite{DBLP:conf/edbt/BrunnerS20} compares different pre-trained LM models for $f()$ while fixing the matcher $M()$. Comparing with~\cite{DBLP:conf/edbt/BrunnerS20} does fit the purpose of Table~\ref{tbl:rpte-expt}.
%
%We have clarified these points in Section~\ref{subsec:rpt-e} ``Preliminary Results''.
%
Moreover, we did not compare with TURL in the ER scenario, because there are several fundamental differences between TURL and \system. %, which are summarized below. 
TURL takes an \emph{entire} table as input to learn contextual representation of the table. Thus, it is designed to serve downstream tasks regarding a \emph{single table}, \eg linking cells in a table to entities in a KB, annotating types of table columns, augmenting table rows/columns. etc. However, it cannot be directly used in the ER scenario that determines whether two tuples across \emph{different tables} are matched or not.
In contrast, \system employs an encoder-decoder architecture to learn representation of tuples or tuple pairs, which can be then fine-tuned to support ER. 

Nevertheless, we compare \system with TURL on the cell filling task, and conduct a new experiment to this end. Please refer to the response to R1W4 \& R1D5 for more details.

%
%\bi
	%\item TURL takes an \emph{entire} table as input to learn contextual representation of the table. Thus, it is designed to serve downstream tasks regarding the tables, \eg, linking cells in a table to entities in a KB, annotating types of table columns, augmenting table rows/columns. etc. However, it cannot be directly used in the ER scenario that determines whether two tuples are matched or not.
	%In contrast, \system employs an encoder-decoder architecture to learn representation of tuples or tuple pairs, which can be then fine-tuned to support ER. 
	%TURL uses an encoder-only architecture; \system employs an encoder-decoder architecture. As has been empirically verified by Google T5~\cite{t5} and BART~\cite{bart}, the encoder-decoder architecture generally outperforms encoder-only architecture for many NLP tasks, yet it provides more flexibility for fine-tuning.
	%
	%\item TURL mainly learns entity representations; \system not only learns tuple representations (the encoder) but also generates values (the decoder).
	%
%	\item TURL cannot do cell filling by its own, and it must be used jointly with a KB (or a collection of web tables) to extract values; \system itself can fill missing values. 
	%
%	More concretely, in our testing, the model of TURL has 1.2 GB and its associated KB (\ie web tables) has 4.7 GB -- these two must be used together to extract and fill values\footnote{We have confirmed this point with the first author of TURL.};
%	the model of \system has 1.6 GB in total without the need of other auxiliary data.
%
%	\item We also conduct another experiment to compare TURL and \system. We extract $1221$ web tables from the dataset used in TURL for pre-training, where each table contains columns regarding \at{city} and \at{country}. Different from TURL, we only use headers as meta-data, and do not assume that the dependency between subject and object columns is given.
%
%	After pre-training, we employ TURL and \system to fill missing values in \at{country} and compare their results. We have the following experimental findings.
%	On the one hand, for $736$ test tables, TURL cannot find subject entity in the KB and thus it returns empty results, while \system can achieve $0.75$ on accuracy. On the other hand, for $1075$ tables, TURL can find subject entities in the KB and obtain $0.64$ on accuracy, while \system achieves $0.69$. Overall, the accuracy scores of TURL and \system are $0.48$ and $0.71$, respectively. The experimental results show that \system can achieve better performance 
%	on cleaning relational tables when no assumptions on column dependency and external knowledge are given.
%\ei

\stab
(3) We have added two discussions on this point.

\bi
	\item The requirement of a high-quality training data as a benchmark in Section~\ref{subsec:rpt-opp} (O2) ``Dirty Data'' and in Section~\ref{sec:conclusion}.
	
	\item The connection with human-in-the-loop systems in Section~\ref{subsec:rpt-opp} (O3) ``An AI-assisted Tool with Human-in-the-loop'', as well as in Section~\ref{subsec:rpt-exp} ``Limitations'' (3).
\ei

\stab
(4) We have added the discussion about the difference of \system with these papers in Section~\ref{subsec:rpt-related} related work, as suggested.
Specifically, TaBERT and TabFact study the \emph{QA tasks} that involve joint reasoning over both free text and structured tables. They take a natural language \emph{utterance} as input and produce a structured query (\eg an SQL query in TaBERT) or a classification result (\eg support or refute in TabFact). To this end, they focus on learning \emph{joint representation} over textual utterance and tabular data with Transformer models and design various pre-training tasks to this end.
Different from these studies, \system focuses on data preparation, such as data cleaning, entity resolution, and so on, and does not study the problem of joint understanding of textual and relational data.


==> response/r3.tex <==
%!TEX root = ../paper.tex
\subsection*{Responses to Reviewer \#3}

\stitle{\fbox{R3D1.}} 
{\em 
Very concrete vision paper. It builds on recent promising results that have shown how deep learning solutions (in particular those based on pretrained transformers) can contribute to solve many important data management problems. 
The discussions on DC and ER are very interesting: the authors identify important challenging open problems that go beyond the standard definition, and highlight interesting research opportunities. 
}


\stitle{[{\em Response to R3D1.}]}
We are naturally glad to hear this comment!

\stitle{\fbox{R3W1.}} 
{\em The information extraction task is just sketched. \\
Unfortunately the IE task is less developed and the discussion is more superficial. Semi-structured data and relational data are mentioned, but actually the problem definition is very narrow and concentrates on extracting spans of text from short descriptions. The research opportunities sketched for this tasks are rather straightforward and seems just an application of NLP solutions to short textual description.
}


\stitle{[{\em Response to R3W1.}]}
We have restructured the paper by using a unified \system model (Section~\ref{sec:rpt-model}) and explained how \system can be fine-tuned for information extraction and data annotation (Section~\ref{sec:finetune}).

Next, we briefly discuss the generality of the above two problems. Given a tuple $x$, we want to have a label $y$ for it. 
We consider the task of {\em Information extraction} if $y$ is extracted from $x$; and {\em data annotation} if $y$ is not from $x$.
%
Apparently, the above two cases can cover a large part of common crowdsourcing tasks, which are considered to be human-easy. 

Besides discussing that \system can be fine-tuned for the above two tasks (Section~\ref{sec:finetune}), we have revised the original discussion about information extraction (Section~\ref{sec:rpt-i}), by describing what other appealing techniques can be used for specific data preparation tasks.

\stitle{\fbox{R3W2.}} 
{\em Examples and benchmarks are mainly focused on the product domain. \\
As a final remark, though I really appreciate that the paper adopts public benchmarks (and encourages their adoption), I am a bit concerned that most of the benchmarks that our community is using are focused on the product domain (it seems that we moved from bibliographic datasets from product datasets). Developing novel benchmarks could be another contribution in the call to arms.}


\stitle{[{\em Response to R3W2.}]}
We fully agree that ``Right Architecture + Good Big Data = State-of-the-art''. The lack of high-quality training data could be a bottleneck. We have added a discussion in Section~\ref{subsec:rpt-opp} (2) ``Dirty Data'', to highlight the importance of good data, such as the Colossal Clean Crawled Corpus (C4) for Text-To-Text-Transfer-Transformer (T5)~\cite{t5}. We have also included this point in Section~\ref{sec:conclusion} ``Call to Arms''.


\stitle{\fbox{R3W3.}} 
{\em What about explainability?. \\
I am surprised that the paper does not mention explainability as an important open problem strictly related to development of any DL solutions. There is a large literature on these topics, but it has been addressed mainly by AI people: solutions are task agnostic and apply to generic classification problems. Developing effective solutions that are related to specific data management tasks is challenging. Our community has recently addressed the problem and there are some interesting yet preliminary contributions on this argument (even by the same authors of this paper). I think is would be worth mentioning the problem. 
}


\stitle{[{\em Response to R3W3.}]}
Explainability is important for deep learning models to be adopted, especially if a system needs to interact with humans. We did not include it in the original submission, because it is complementary to the techniques discussed in this paper. 
We have added a discussion at Section~\ref{subsec:rpt-opp} (O3) ``An AI-assisted Tool with Human-in-the-loop'' to emphasize the importance of model explainablity, especially when having human-in-the-loop. 
